RBO Hand 3 -- A Platform for Soft Dexterous Manipulation

We present the RBO Hand 3, a highly capable and versatile anthropomorphic soft hand based on pneumatic actuation. The RBO Hand 3 is designed to enable dexterous manipulation, to facilitate transfer of insights about human dexterity, and to serve as a robust research platform for extensive real-world experiments. It achieves these design goals by combining many degrees of actuation with intrinsic compliance, replicating relevant functioning of the human hand, and by combining robust components in a modular design. The RBO Hand 3 possesses 16 independent degrees of actuation, implemented in a dexterous opposable thumb, two-chambered fingers, an actuated palm, and the ability to spread the fingers. In this work, we derive the design objectives that are based on experimentation with the hand's predecessors, observations about human grasping, and insights about principles of dexterity. We explain in detail how the design features of the RBO Hand 3 achieve these goals and evaluate the hand by demonstrating its ability to achieve the highest possible score in the Kapandji test for thumb opposition, to realize all 33 grasp types of the comprehensive GRASP taxonomy, to replicate common human grasping strategies, and to perform dexterous in-hand manipulation.

==> pdf_submission_log.tex <==
Successfully uploaded puhlmann-21-T-RO.pdf

2021-09-06 05:43:26	ProcessID	798	
2021-09-06 05:43:26	Profile	/home/papercept/ras.papercept.net/www/journals/tro/scripts/New_Process_plan.kfpx	
2021-09-06 05:43:26	Input	/home/common/www/conferences/spool/X7T5WIyQE8.pdf	
2021-09-06 05:43:26	Pages	15	
2021-09-06 05:43:26	Progress	1	%
2021-09-06 05:43:26	Step	Profile	HK Remove glyphs with invalid encoding
2021-09-06 05:43:27	Progress	7	%
2021-09-06 05:43:27	Progress	17	%
2021-09-06 05:43:27	Progress	18	%
2021-09-06 05:43:27	Progress	19	%
2021-09-06 05:43:27	Progress	20	%
2021-09-06 05:43:27	Progress	21	%
2021-09-06 05:43:27	Progress	22	%
2021-09-06 05:43:27	Progress	23	%
2021-09-06 05:43:27	Progress	24	%
2021-09-06 05:43:27	Progress	25	%
2021-09-06 05:43:27	Progress	26	%
2021-09-06 05:43:27	Progress	27	%
2021-09-06 05:43:27	Progress	28	%
2021-09-06 05:43:27	Progress	29	%
2021-09-06 05:43:27	Progress	30	%
2021-09-06 05:43:27	Progress	31	%
2021-09-06 05:43:27	Progress	32	%
2021-09-06 05:43:27	Progress	33	%
2021-09-06 05:43:27	Progress	34	%
2021-09-06 05:43:27	Progress	35	%
2021-09-06 05:43:27	Progress	36	%
2021-09-06 05:43:27	Progress	37	%
2021-09-06 05:43:27	Progress	38	%
2021-09-06 05:43:27	Progress	48	%
2021-09-06 05:43:27	Progress	49	%
2021-09-06 05:43:27	Progress	50	%
2021-09-06 05:43:27	Progress	54	%
2021-09-06 05:43:27	Progress	55	%
2021-09-06 05:43:27	Progress	57	%
2021-09-06 05:43:27	Progress	58	%
2021-09-06 05:43:27	Progress	59	%
2021-09-06 05:43:27	Progress	61	%
2021-09-06 05:43:27	Progress	62	%
2021-09-06 05:43:27	Progress	63	%
2021-09-06 05:43:27	Progress	65	%
2021-09-06 05:43:27	Progress	66	%
2021-09-06 05:43:27	Progress	67	%
2021-09-06 05:43:27	Progress	69	%
2021-09-06 05:43:27	Progress	70	%
2021-09-06 05:43:27	Progress	71	%
2021-09-06 05:43:27	Progress	72	%
2021-09-06 05:43:27	Progress	74	%
2021-09-06 05:43:27	Progress	75	%
2021-09-06 05:43:27	Progress	76	%
2021-09-06 05:43:27	Progress	78	%
2021-09-06 05:43:27	Progress	79	%
2021-09-06 05:43:27	Progress	80	%
2021-09-06 05:43:27	Progress	82	%
2021-09-06 05:43:27	Progress	83	%
2021-09-06 05:43:27	Progress	84	%
2021-09-06 05:43:27	Progress	86	%
2021-09-06 05:43:27	Progress	87	%
2021-09-06 05:43:27	Progress	88	%
2021-09-06 05:43:27	Progress	90	%
2021-09-06 05:43:27	Progress	91	%
2021-09-06 05:43:27	Progress	92	%
2021-09-06 05:43:27	Progress	100	%
2021-09-06 05:43:27	Summary	Corrections	0
2021-09-06 05:43:27	Summary	Errors	0
2021-09-06 05:43:27	Summary	Warnings	0
2021-09-06 05:43:27	Summary	Infos	0
2021-09-06 05:43:27	Step	Fixup	Downsample bitmap images to 300 ppi if above 450 ppi
2021-09-06 05:43:27	Summary	Corrections	0
2021-09-06 05:43:27	Summary	Errors	0
2021-09-06 05:43:27	Summary	Warnings	0
2021-09-06 05:43:27	Summary	Infos	0
2021-09-06 05:43:27	Step	Profile	HK Embedded files check
2021-09-06 05:43:27	Summary	Corrections	0
2021-09-06 05:43:27	Summary	Errors	0
2021-09-06 05:43:27	Summary	Warnings	0
2021-09-06 05:43:27	Summary	Infos	0
2021-09-06 05:43:27	Step	Profile	HK Embedded Postscript check
2021-09-06 05:43:27	Summary	Corrections	0
2021-09-06 05:43:27	Summary	Errors	0
2021-09-06 05:43:27	Summary	Warnings	0
2021-09-06 05:43:27	Summary	Infos	0
2021-09-06 05:43:27	Step	Profile	HK Nonembedded check
2021-09-06 05:43:27	Summary	Corrections	0
2021-09-06 05:43:27	Summary	Errors	0
2021-09-06 05:43:27	Summary	Warnings	0
2021-09-06 05:43:27	Summary	Infos	0
2021-09-06 05:43:27	Step	Profile	HK Not subset check
2021-09-06 05:43:28	Summary	Corrections	0
2021-09-06 05:43:28	Summary	Errors	0
2021-09-06 05:43:28	Summary	Warnings	0
2021-09-06 05:43:28	Summary	Infos	0
2021-09-06 05:43:28	Step	Profile	HK Version below 1.4 check
2021-09-06 05:43:28	Summary	Corrections	0
2021-09-06 05:43:28	Summary	Errors	0
2021-09-06 05:43:28	Summary	Warnings	0
2021-09-06 05:43:28	Summary	Infos	0
2021-09-06 05:43:28	Output	/home/common/www/conferences/spool/X7T5WIyQE8.pdf.pdf	
2021-09-06 05:43:28	Finished	/home/common/www/conferences/spool/X7T5WIyQE8.pdf	
2021-09-06 05:43:28	Duration	00:02	
Successfully moved the pdf file to the temporary directory



Bookmarks and annotations were successfully removed

The pdf file is ready to be submitted

